Technical Report: A Toolkit for Runtime Detection of Userspace Implants

This paper presents the Userspace Integrity Measurement Toolkit (USIM Toolkit), a set of integrity measurement collection tools capable of detecting advanced malware threats, such as memory-only implants, that evade many traditional detection tools. Userspace integrity measurement validates that a platform is free from subversion by validating that the current state of the platform is consistent with a set of invariants. The invariants enforced by the USIM Toolkit are carefully chosen based on the expected behavior of userspace, and key behaviors of advanced malware. Userspace integrity measurement may be combined with existing filesystem and kernel integrity measurement approaches to provide stronger guarantees that a platform is executing the expected software and that the software is in an expected state.

==> motivation.tex <==
\section{Motivation}
\label{sec:motivation}

Userspace measurement is intended to detect malicious modifications to
a platform's execution environment. To implement malicious
functionality while remaining stealthy, advanced malware frequently
manipulates this execution environment in distinct ways. Userspace
measurement is focused on revealing these modifications by gathering
evidence of the current state of the platform and comparing this
evidence with a representation of the ways well behaved software
interacts with its environment.

File system hashing is a common form of userspace integrity
measurement. Many tools exist that compute cryptographic hashes of all
or a subset of the files in a filesystem. These hashes can be used
to determine if any files have changed since the last measurement, or
they can be compared to use-case specific whitelists or blacklists. The first
widely known tool in this family is Tripwire\cite{tripwire}, which
dates back to the 1990s. More modern approaches such as the Integrity
Measurement Architecture (IMA)\cite{ima} can make use of a Trusted
Platform Module (TPM)\cite{tpm} to provide a root of trust for the
measurement. File system hashing is an important form of userspace
integrity measurement but is insufficient as it is unable to detect
malware that (a) does not exist in the filesystem or (b) exists in
locations of the filesystem with unconstrained expected hashes (e.g.,
user home directories). 


